An update on site search activities for SWGO

The Southern Wide-field Gamma-ray Observatory (SWGO) is a project by scientists and engineers from 14 countries and 78 institutions to design and build the first wide-field, ground-based gamma-ray observatory in the Southern Hemisphere, with high duty cycle and covering an energy range rom hundreds of GeV to the PeV scale. The observatory will cover the Southern sky and aims to map the Galaxy's large-scale emission, as well as detecting transient and variable phenomena. The host sites under consideration are at a minimum altitude of 4400 m.a.s.l. and comprise two types: flat plateaus of at least 1 km$^{2}$ for the installation of an array of tank-based water Cherenkov detectors (WCD), or large natural lakes for the direct deployment of WCD units. Four South American countries proposed excellent sites to host the observatory meeting these requirements. Argentina proposed two locations in the Salta province, Bolivia presented one site in Chacaltaya, Chile two locations within the Atacama Astronomical Park, and Peru two ground-based locations in the Arequipa district as well as lakes in the Cuzco region. The SWGO collaboration is currently conducting a site characterization study, gathering all the necessary information for site shortlisting and final site selection by the end of 2023. The process has reached the shortlisting phase, in which primary and backup sites for each country have been identified. The primary sites were visited by a team of experts from the collaboration, to investigate and validate the proposed site characteristics. Here we present an update on these site selection activities.

==> authorlist_SWGO.tex <==
\title{
    The SWGO Collaboration
\bigskip
\bigskip
\bigskip
\bigskip
\bigskip
}



\author[1,2]{P.~Abreu}
\author[3]{A.~Albert}
\author[4]{R.~Alfaro}
\author[5]{A.~Alfonso}
\author[6]{C.~Álvarez}
\author[7]{Q.~An}
\author[8]{E.~O.~Angüner}
\author[9]{C.~Arcaro}
\author[6]{R.~Arceo}
\author[10]{S.~Arias}
\author[11]{H.~Arnaldi}
\author[1,2]{P.~Assis}
\author[12]{H.~A.~Ayala Solares}
\author[13]{A.~Bakalova}
\author[14,15]{U.~Barres de Almeida}
\author[9,16]{I.~Batkovic}
\author[17]{J.~Bazo}
\author[18,19]{J.~Bellido}
\author[4]{E.~Belmont}
\author[20]{S.~Y.~BenZvi}
\author[21]{A.~Bernal}
\author[22]{W.~Bian}
\author[23]{C.~Bigongiari }
\author[9,16]{E.~Bottacini}
\author[1,2]{P.~Brogueira}
\author[24]{T.~Bulik}
\author[9,16]{G.~Busetto}
\author[6]{K.~S.~Caballero-Mora}
\author[25,26]{P.~Camarri}
\author[27]{S.~Campos}
\author[7]{W.~Cao}
\author[7]{Z.~Cao}
\author[28]{Z.~Cao}
\author[21]{T.~Capistrán}
\author[23]{M.~Cardillo}
\author[29]{E.~Carquin}
\author[30]{A.~Carramiñana}
\author[31]{C.~Castromonte}
\author[28]{J.~Chang}
\author[32]{O.~Chaparro}
\author[22]{S.~Chen}
\author[33,34]{M.~Chianese}
\author[35,36]{A.~Chiavassa}
\author[13]{L.~Chytka}
\author[33,34]{R.~Colallillo}
\author[1,2]{R.~Conceição}
\author[37,38]{G.~Consolati}
\author[39]{R.~Cordero}
\author[1,2]{P.~J.~Costa}
\author[40]{J.~Cotzomi}
\author[41]{S.~Dasso}
\author[9,16]{A.~De Angelis}
\author[42]{P.~Desiati}
\author[36]{F.~Di Pierro}
\author[25]{G.~Di Sciascio}
\author[42]{J.~C.~Díaz Vélez}
\author[29]{C.~Dib}
\author[3]{B.~Dingus}
\author[43]{J.~Djuvsland}
\author[44]{C.~Dobrigkeit }
\author[1, 45]{L.~M.~Domingues Mendes}
\author[9]{T.~Dorigo}
\author[9,16]{M.~Doro}
\author[14]{A.~C.~dos Reis}
\author[42]{M.~Du Vernois}
\author[5]{M.~Echiburú}
\author[46]{D.~Elsaesser}
\author[2,46]{K.~Engel}
\author[48]{T.~Ergin}
\author[5]{F.~Espinoza}
\author[42]{K.~Fang}
\author[49]{F.~Farfán Carreras}
\author[38,50]{A.~Fazzi}
\author[51]{C.~Feng}
\author[23]{M.~Feroci}
\author[21]{N.~Fraija}
\author[21]{S.~Fraija}
\author[16]{A.~Franceschini}
\author[14]{G.~F.~Franco}
\author[52]{S.~Funk}
\author[10]{S.~Garcia}
\author[53]{J.~A.~García-González}
\author[21]{F.~Garfias}
\author[22]{G.~Giacinti}
\author[1,2]{L.~Gibilisco}
\author[52]{J.~Glombitza}
\author[43]{H.~Goksu}
\author[54]{G.~Gong}
\author[1,2]{B.~S.~González}
\author[21]{M.~M.~Gonzalez}
\author[47]{J.~Goodman}
\author[28]{M.~Gu}
\author[33,34]{F.~Guarino}
\author[55]{S.~Gupta}
\author[43]{F.~Haist}
\author[29]{H.~Hakobyan}
\author[56]{G.~Han}
\author[57]{P.~Hansen}
\author[3]{J.~P.~Harding}
\author[5]{J.~Helo}
\author[58]{I.~Herzog}
\author[6]{H.~d.~Hidalgo}
\author[43]{J.~Hinton}
\author[51]{K.~Hu}
\author[47]{D.~Huang}
\author[59]{P.~Huentemeyer}
\author[6]{F.~Hueyotl-Zahuantitla}
\author[21]{A.~Iriarte}
\author[60]{J.~Isaković}
\author[61]{A.~Isolia}
\author[52]{V.~Joshi}
\author[13]{J.~Juryšek}
\author[22]{S.~Kaci}
\author[62]{D.~Kieda}
\author[23]{F.~La Monaca}
\author[1]{G.~La Mura}
\author[52]{R.~G.~Lang}
\author[27]{R.~Laspiur}
\author[34]{L.~Lavitola}
\author[63]{J.~Lee}
\author[52]{F.~Leitl}
\author[23]{L.~Lessio }
\author[28]{C.~Li}
\author[7]{J.~Li}
\author[28]{K.~Li}
\author[22]{T.~Li}
\author[25,26]{B.~Liberti}
\author[64]{S.~Lin}
\author[51]{D.~Liu}
\author[28]{J.~Liu}
\author[65]{R.~Liu}
\author[66,67]{F.~Longo}
\author[22]{Y.~Luo}
\author[68]{J.~Lv}
\author[38,50]{E.~Macerata}
\author[3]{K.~Malone}
\author[13]{D.~Mandat}
\author[60]{M.~Manganaro}
\author[38,50]{M.~Mariani}
\author[57]{A.~Mariazzi}
\author[9,16]{M.~Mariotti}
\author[43]{T.~Marrodan}
\author[32]{J.~Martinez}
\author[69]{H.~Martínez-Huerta}
\author[5]{S.~Medina}
\author[70]{D.~Melo}
\author[2]{L.~F.~Mendes}
\author[72]{E.~Meza}
\author[9]{D.~Miceli}
\author[25]{S.~Miozzi}
\author[52]{A.~Mitchell}
\author[36,71]{A.~Molinario}
\author[6]{O.~G.~Morales-Olivares}
\author[40]{E.~Moreno }
\author[25,26]{A.~Morselli}
\author[38,50]{E.~Mossini}
\author[12]{M.~Mostafá}
\author[23]{F.~Muleri}
\author[9,16]{F.~Nardi}
\author[35,36]{A.~Negro}
\author[73]{L.~Nellen}
\author[13]{V.~Novotny}
\author[66,67]{E.~Orlando}
\author[21]{M.~Osorio}
\author[72]{L.~Otiniano}
\author[35,36]{M.~Peresano}
\author[23]{G.~Piano}
\author[41]{A.~Pichel}
\author[9,16]{M.~Pihet}
\author[1,2]{M.~Pimenta}
\author[9,16]{E.~Prandini}
\author[7]{J.~Qin}
\author[72,74]{E.~Quispe}
\author[75]{S.~Rainò}
\author[21]{E.~Rangel}
\author[55]{A.~Reisenegger}
\author[43]{H.~Ren}
\author[60]{F.~Reščić}
\author[43]{B.~Reville}
\author[76]{C.~D.~Rho}
\author[77]{M.~Riquelme}
\author[25]{G.~Rodriguez Fernandez}
\author[63]{Y.~Roh}
\author[49]{G.~E.~Romero}
\author[34]{B.~Rossi}
\author[41]{A.~C.~Rovero}
\author[43]{E.~Ruiz-Velasco}
\author[27]{G.~Salazar}
\author[72]{J.~Samanes}
\author[70]{F.~Sanchez}
\author[4]{A.~Sandoval}
\author[78]{M.~Santander}
\author[25,26]{R.~Santonico}
\author[14]{G.~L.~P.~Santos}
\author[33,34]{N.~Saviano}
\author[47]{M.~Schneider}
\author[52]{M.~Schneider}
\author[79]{H.~Schoorlemmer}
\author[4]{J.~Serna-Franco}
\author[27]{V.~Serrano}
\author[47]{A.~Smith}
\author[63]{Y.~Son}
\author[80]{O.~Soto}
\author[62]{R.~W.~Springer}
\author[81]{L.~A.~Stuani}
\author[51]{H.~Sun}
\author[22]{R.~Tang}
\author[7]{Z.~Tang}
\author[29]{S.~Tapia}
\author[23]{M.~Tavani}
\author[60]{T.~Terzić}
\author[58]{K.~Tollefson}
\author[1,2]{B.~Tomé}
\author[30]{I.~ Torres}
\author[22]{R.~Torres-Escobedo}
\author[36,71]{G.~C.~Trinchero}
\author[59]{R.~Turner}
\author[80]{P.~Ulloa}
\author[33,34]{L.~Valore}
\author[52]{C.~van Eldik}
\author[57]{I.~Vergara}
\author[82]{A.~Viana}
\author[13]{J.~Vícha}
\author[35,36]{C.~F.~Vigorito}
\author[23]{V.~Vittorini}
\author[51]{B.~Wang}
\author[43]{J.~Wang}
\author[28]{L.~Wang}
\author[59]{X.~Wang}
\author[65]{X.~Wang}
\author[83]{X.~Wang}
\author[22]{Z.~Wang}
\author[33,34]{M.~Waqas}
\author[63]{I.~J.~Watson}
\author[43]{F.~Werner}
\author[43]{R.~White}
\author[84]{C.~Wiebusch}
\author[47]{E.~J.~Willox}
\author[43]{F.~Wohlleben}
\author[28]{S.~Wu}
\author[28]{S.~Xi}
\author[28]{G.~Xiao}
\author[64]{L.~Yang}
\author[7]{R.~Yang}
\author[18]{R.~Yanyachi }
\author[28]{Z.~Yao}
\author[85]{D.~Zavrtanik}
\author[22]{H.~Zhang}
\author[65]{H.~Zhang}
\author[86]{S.~Zhang}
\author[28]{X.~Zhang}
\author[68]{Y.~Zhang}
\author[28]{J.~Zhao}
\author[7]{L.~Zhao}
\author[22]{H.~Zhou}
\author[51]{C.~Zhu}
\author[87]{P.~Zhu}
\author[28]{X.~Zuo}


\affil[1]{Laborat\'{o}rio de Instrumenta\c{c}\~ao de F\'{\i}sica Experimental de Part\'{\i}culas - LIP, Av.~Prof.~Gama Pinto, 2, 1649-003 Lisboa, Portugal}
\affil[2]{Departamento de F\'{\i}sica,  Instituto Superior T\'ecnico, Universidade de Lisboa, Av.~Rovisco Pais 1, 1049-001 Lisboa, Portugal}
\affil[3]{Physics Division, Los Alamos National Laboratory, Los Alamos, NM, USA}
\affil[4]{Instituto de F\' isica, Universidad Nacional Aut\'onoma de M\'exico, Circuito de la Investigaci\'on Cient\'ifica, C.U., A.~Postal 70-364, 04510 Cd.~de M\'exico,  M\'exico}
\affil[5]{Universidad de La Serena, Chile}
\affil[6]{Facultad de Ciencias en F\'isica y Matem\'aticas, Universidad Aut\'onoma de Chiapas, C.~P.~29050, Tuxtla Guti\'errez,  Chiapas, M\'exico}
\affil[7]{School of physical science, University of Science and Technology of China, 96 Jinzhai Road, Hefei, Anhui 230026, China}
\affil[8]{TÜBİTAK Research Institute for Fundamental Sciences, 41470 Gebze, Turkey}
\affil[9]{INFN - Sezione di Padova, I-35131, Padova, Italy }
\affil[10]{Universidad Nacional de San Antonio Abad del Cusco, Av.~de la Cultura, Nro.~733, Cusco - Perú}
\affil[11]{Centro Atómico Bariloche (CNEA-CONICET-IB/UNCuyo), Av.~E.~Bustillo 9500, (8400) San Carlos de Bariloche, Rio Negro, Argentina}
\affil[12]{Department of Physics, Pennsylvania State University, University Park, PA, USA}
\affil[13]{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}
\affil[14]{Centro Brasileiro de Pesquisas Físicas (CBPF), Rua Dr.~Xavier Sigaud 150, 22290-180 Rio de Janeiro, Brasil}
\affil[15]{Universidade de São Paulo, Instituto de Astronomia, Geofísica e Ciências Atmosféricas, Departamento de Astronomia, Rua do Matão 1226, 05508-090 São Paulo, Brasil}
\affil[16]{Università di Padova, I-35131, Padova, Italy}
\affil[17]{Pontificia Universidad Católica del Perú,  Av.~Universitaria 1801, San Miguel, 15088, Lima, Perú}
\affil[18]{Universidad Nacional de San Agustin de Arequipa, Santa Catalina Nro.~117.~Arequipa}
\affil[19]{University of Adelaide, Adelaide, S.A., Australia }
\affil[20]{Department of Physics and Astronomy, University of Rochester, Rochester, NY, USA}
\affil[21]{Instituto de Astronom\' ia, Universidad Nacional Aut\'onoma de M\'exico, Circuito Exterior, C.U., A.~Postal 70-264, 04510 Cd.~de M\'exico,  M\'exico}
\affil[22]{Tsung-Dao Lee Institute \& School of Physics and Astronomy, Shanghai Jiao Tong University, 520 Shengrong Road, Shanghai 201210, China}
\affil[23]{Istituto Nazionale Di Astrofisica (INAF), Roma, Italy}
\affil[24]{Astronomical Observatory Warsaw University, 00-478 Warsaw, Poland}
\affil[25]{INFN, Roma Tor Vergata, Italy }
\affil[26]{Department of Physics, University of Roma Tor Vergata, Viale della Ricerca Scientifica 1, I-00133 Roma, Italy}
\affil[27]{Facultad de Ciencias Exactas, Universidad Nacional de Salta, Avda.~Bolivia 5150, A4408FVY, Salta, Argentina}
\affil[28]{Institute of High Energy Physics, Chinese Academy of Science, 19B Yuquan Road, Shijingshan District, Beijing 100049, China}
\affil[29]{CCTVal, Universidad Tecnica Federico Santa Maria, Chile}
\affil[30]{Instituto Nacional de Astrofísica, Óptica y Electrónica, Puebla, Mexico}
\affil[31]{Universidad Nacional de Ingeniería, Av.~Túpac Amaru 210 - Rímac.~Apartado 1301, Lima Perú}
\affil[32]{Centro de Investigaci\'on en Computaci\'on, Instituto Polit\'ecnico Nacional, Ciudad de M\'exico, Mexico}
\affil[33]{Università di Napoli “Federico II”, Dipartimento di Fisica “Ettore Pancini”, Napoli, Italy}
\affil[34]{INFN, Sezione di Napoli, Napoli, Italy}
\affil[35]{Università degli Studi di Torino, I-10125 Torino, Italy}
\affil[36]{INFN, Sezione di Torino, Torino, Italy}
\affil[37]{Politecnico di Milano, Dipartimento di Scienze e Tecnologie Aerospaziali, Milano, Italy}
\affil[38]{INFN, sezione di Milano, Milano, Italy}
\affil[39]{Departamento de Física, Universidad de Santiago de Chile, Chile}
\affil[40]{Facultad de Ciencias Físico Matemáticas, Benemérita Universidad Autónoma de Puebla,  Av.~San Claudio y 18 Sur, Ciudad Universitaria 72570, Puebla, Mexico.}
\affil[41]{Instituto de Astronomía y Física del Espacio (IAFE (CONICET-UBA)), Ciudad Universitaria, CABA, Argentina}
\affil[42]{Department of Physics, University of Wisconsin-Madison, Madison, WI, USA}
\affil[43]{Max-Planck-Institut für Kernphysik, Saupfercheckweg 1, 69117 Heidelberg, Germany}
\affil[44]{Departamento de Raios Cósmicos e Cronologia, Instituto de Física "Gleb Wataghin", Universidade Estadual de Campinas, C.P.~6165, 13083-970 Campinas, Brasil }
\affil[45]{Centro Federal de Educação Tecnológica Celso Suckow da Fonseca (CEFET), Rio de Janeiro, Brasil}
\affil[46]{Technische Universität Dortmund, D-44221 Dortmund, Germany}
\affil[47]{Department of Physics, University of Maryland, College Park, MD, USA}
\affil[48]{Middle East Technical University, Northern Cyprus Campus, 99738 Kalkanli via Mersin 10, Turkey}
\affil[49]{Instituto Argentino de Radioastronomía (CONICET, CIC, UNLP), Camino Gral.~Belgrano Km 40, Berazategui, Argentina}
\affil[50]{Politecnico di Milano, Dipartimento di Energia, Milano, Italy}
\affil[51]{Key Laboratory of Particle Physics and Particle Irradiation (MOE), Institute of Frontier and Interdisciplinary Science, Shandong University, Qingdao, Shandong 266237, China}
\affil[52]{Friedrich-Alexander-Universität Erlangen-Nürnberg, Erlangen Centre for Astroparticle Physics, Nikolaus-Fiebiger-Str.~2, D 91058 Erlangen, Germany}
\affil[53]{Tecnologico de Monterrey, Escuela de Ingeniería y Ciencias, Ave.~Eugenio Garza Sada 2501, Monterrey, N.L., Mexico, 64849}
\affil[54]{Dept.~of Engineering Physics, Tsinghua University, 1 Tsinghua Yuan, Haidian District, Beijing 100084, China}
\affil[55]{Universidad Metropolitana de Ciencias de la Educación (UMCE), Chile}
\affil[56]{School of Mechanical Engineering and Electronic Information, China University of Geosciences, Wuhan, Hubei 430074, China}
\affil[57]{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}
\affil[58]{Department of Physics and Astronomy, Michigan State University, East Lansing, MI, USA}
\affil[59]{Michigan Technological University, Houghton, Michigan, 49931, USA}
\affil[60]{University of Rijeka, Faculty of Physics, 51000 Rijeka, Croatia}
\affil[61]{Università di Catania, Catania, Italy}
\affil[62]{Department of Physics and Astronomy, University of Utah, Salt Lake City, UT, USA}
\affil[63]{University of Seoul, Seoul, Rep.~of Korea}
\affil[64]{School of Physics and Astronomy, Sun Yat-sen University, Zhuhai, Guangdong 519082, China}
\affil[65]{School of Astronomy and Space Science, Nanjing University, Xianlin Avenue 163, Qixia District, Nanjing, Jiangsu 210023, China}
\affil[66]{Dipartimento di Fisica, Università degli Studi di Trieste, Trieste, Italy}
\affil[67]{INFN - Sezione di Trieste,  via Valerio 2, I - 34149 ,Trieste, Italy}
\affil[68]{Aerospace Information Research Institute, Chinese Academy of Science, 9 Dengzhuang South Road, Haidian District, Beijing 100094, China}
\affil[69]{Departamento de Física y Matemáticas, Universidad de Monterrey, Av.~Morones Prieto 4500, 66238, San Pedro Garza Garc\'ia NL, M\'exico}
\affil[70]{Instituto de Tecnologías en Detección y Astropartículas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affil[71]{Instituto Nazionale Di Astrofisica (INAF), Torino, Italy}
\affil[72]{Comisión Nacional de Investigación y Desarrollo Aeroespacial, Perú}
\affil[73]{Instituto de Ciencias Nucleares, Universidad Nacional Aut\'onoma de M\'exico, Circuito Exterior, C.U., A.~Postal 70-543, 04510 Cd.~de M\'exico,  M\'exico}
\affil[74]{Universidad Nacional de Moquegua}
\affil[75]{Università degli Studi di Bari Aldo Moro, Italy}
\affil[76]{Department of Physis, Sungkyunkwan University, Suwon, South Korea}
\affil[77]{Universidad de Chile, Chile}
\affil[78]{Department of Physics and Astronomy, University of Alabama, Tuscaloosa, Alabama, 35487, USA}
\affil[79]{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affil[80]{Unidade Acadêmica de Física, Universidade Federal de Campina Grande, Av.~Aprígio Veloso 882, CY2, 58.429-900 Campina Grande, Brasil}
\affil[81]{Instituto de F\'isica de S\~ao Carlos, Universidade de S\~ao Paulo, Av.~Trabalhador S\~ao-carlense 400, S\~ao Carlos, Brasil}
\affil[82]{School of Integrated Circuit, Ludong University, 186 Hongqi Middle Road, Zhifu District, Yantai, Shandong, China}
\affil[83]{III.~Physics Institute A, RWTH Aachen University, Templergraben 56, D-52062 Aachen, Germany }
\affil[84]{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}
\affil[85]{College of Engineering, Hebei Normal University, 20 South Second Ring East Road, Shijiazhuang, Hebei, China}
\affil[86]{School of mechanical engineering, University of Science and Technology Beijing, 30 Xueyuan Road, Haidian District, Beijing 100083, China}

